Reinforcement Learning-based Adaptive Mitigation of Uncorrected DRAM Errors in the Field

Scaling to larger systems, with current levels of reliability, requires cost-effective methods to mitigate hardware failures. One of the main causes of hardware failure is an uncorrected error in memory, which terminates the current job and wastes all computation since the last checkpoint. This paper presents the first adaptive method for triggering uncorrected error mitigation. It uses a prediction approach that considers the likelihood of an uncorrected error and its current potential cost. The method is based on reinforcement learning, and the only user-defined parameters are the mitigation cost and whether the job can be restarted from a mitigation point. We evaluate our method using classical machine learning metrics together with a cost-benefit analysis, which compares the cost of mitigation actions with the benefits from mitigating some of the errors. On two years of production logs from the MareNostrum supercomputer, our method reduces lost compute time by 54% compared with no mitigation and is just 6% below the optimal Oracle method. All source code is open source.

==> 90-Artifact.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Description}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

This paper presents the first adaptive method for triggering DRAM uncorrected error (UE) mitigation. It uses a reinforcement learning (RL) approach that considers the likelihood of an uncorrected error, its current potential cost and the cost of performing a mitigation.
The accompanying artifact provides the code and data necessary for training and evaluating the reinforcement learning agent and other machine learning strategies employed in the paper.

As depicted in Figure~\ref{fig:agent-and-environment}, the RL agent addresses the MDP challenge by interacting with the environment. In our approach, which is based on historical data, the environment retrieves UEs, events, and job state from the logs. In an operational system, this data would be collected from monitoring daemons and the workload manager. The environment communicates the state to the agent, which inputs state features into the neural network to ascertain the optimal action, either to initiate a mitigation or not. A dueling double deep Q-learning neural network is implemented to avert overestimation of action values and to enhance policy learning.

During the training phase, each episode represents a "run" of the agent in its environment, from an initial to a terminal state. In this context, a single node is randomly selected, and the episode proceeds from the beginning to the end of the split (Section~\ref{ssec:time-series-xval}), encompassing all events on that node. A series of jobs is arbitrarily chosen to execute on the node, with weighting based on the number of nodes on which the jobs run, ensuring the proper job distribution. Throughout training, the agent refines its future actions by maximizing the reward derived from its current experience.

The evaluation phase, which includes validation and testing, is crucial in assessing the agent's performance and generalization. During validation, the agent's model is fine-tuned on a portion of the dataset, separate from the training data, to prevent overfitting and optimize hyperparameters. During testing, the agent’s model is evaluated on the last portion of the dataset, separate from training and validation data, testing the agent’s ability to perform in unseen situations. The performance metrics obtained from the validation and testing phases offer valuable insights into the agent's efficiency and robustness.

The project is developed in Python 3.6.4 with the following libraries: numpy 3.6.4, pandas 1.0.1, sklearn 0.22.1, stable\_baselines3 0.11.0a7, and matplotlib 3.5.3.

We release synthetic logs, covering a similar 26-month period as the experiments in the paper:

\begin{itemize}
	\item Feature logs corresponding to the features listed in Table~\ref{tab:Features}. These are used by the models for predicting possible upcoming UEs.
	\item DRAM UEs, detailing DRAM id, time and error type (over-temperature vs ECC)
%	The time between events follows an exponential Weibull distribution, separately for over-temperature and ECC errors, which \fixme{seems to be / is / has proved to be...} an excellent match to the real DRAM UE distribution~\cite{Schroeder:TDSC2010}.
	are the same logs shared by Boixaderas et al.~\cite{boixaderas2020cost} based on the same system and time period.
	\item Job distribution specifies the jobs start time, duration, and the total number of nodes used.
\end{itemize}

% \ib{Should we be more explicit that the experiments in the paper cannot be reproduced with this data?}


%This paper presents the first adaptive method for triggering DRAM uncorrected error (UE) mitigation. It uses a reinforcement learning (RL) approach that considers the likelihood of an uncorrected error, its current potential cost and the cost of performing a mitigation. The accompanying artifact provides the code and data necessary for training and evaluating reinforcement learning agents in the context of DRAM uncorrected error mitigation.
%
%The raw workload and error logs are considered to be sensitive and confidential information, thus they cannot be publicly shared. Instead \fixme{to help the community...?}, we release synthetic logs covering the same 26-month period:
%
%\ib{We may decide to not include the explanations of how the logs are generated.}
%
%\begin{itemize}
%	\item Feature logs corresponding to the features listed in Table~\ref{tab:Features}. These are used by the models for predicting possible upcoming UEs. \fixme{How do we generate them?}
%	\item DRAM UEs, detailing DRAM id, time and error type (over-temperature vs ECC). The time between events follows an exponential Weibull distribution, separately for over-temperature and ECC errors, which \fixme{seems to be / is / has proved to be...} an excellent match to the real DRAM UE distribution~\cite{Schroeder:TDSC2010}. These are the same logs shared by Boixaderas et al.~\cite{boixaderas2020cost} based on the same system and time period.
%	\item Job distributions for each node, specifying the jobs start time, duration, and the total number of nodes used. \fixme{How do we generate them?}
%\end{itemize}
%
%\ib{Should we be more explicit that the experiments in the paper cannot be reproduced with this data?}
%
%%%%%%%%%%% 
%
%Following the overall approach illustrated in Figure~\ref{fig:agent-and-environment}, we provide several programs for training and evaluating the RL models:
%
%\begin{itemize}
%	\item \textbf{Environment}: encodes the features, UEs, and jobs derived from the logs and transfers this state information to the agent, which then performs an action. Following the agent's decision, the environment computes the reward (as described in Section~\ref{ssec:reward}) based on the mitigation and UE costs, and provides this feedback to the agent.
%	\item \textbf{Agent}: supplies the state information given by the environment to the neural network, which subsequently determines whether the system should initiate a mitigation action. As described in Section~\ref{sec:background}, the agent employs two approaches during training: dueling double deep Q-network and prioritized experience replay.
%	\item \textbf{Evaluation}: evaluates the performance of a model with the validation and test data.
%	\item \textbf{Main}: creates the environment and the agent with the specified parameters, such as mitigation cost or time period. It then proceeds to train and evaluate the model.
%\end{itemize}


\subsection{Reproducibility of the experiments}

The raw workload and error logs (Section~\ref{sec:Environment}) are considered
to be sensitive and confidential information that cannot be publicly shared.
We therefore release synthetic logs, covering a similar period, which can be
used to verify that the installation is working properly and assist in applying
the method to other systems.  We provide multiple scripts for reproducing the
workflow of the experiments reported in the paper:

\begin{enumerate}
	\item Train and evaluate multiple agents with time series cross-validation (Section~\ref{ssec:time-series-xval}), which separates the features dataset into independent splits. For each split, train a set of agents with different hyperparameters, and subsequently evaluate them with the validation and test sets.
	\item For each split, select the best performing agent on validation data. These are the agents which would be realistically chosen in a production environment. The overall performance is determined by the test performance of these agents.
	\item Optionally, evaluate the performance of other strategies (Section \ref{ssec:approaches}): Never-mitigate, Always-mitigate, Oracle, SC20-RF, and Myopic-RF.
	\item Generate a bar chart resembling Figure~\ref{fig:total-costs-mitigation}. The resulting plot enables the visualization and comparison of the overall performance across the different strategies.
\end{enumerate}

The time required for training multiple agents and calculating the performance of the six strategies with the synthetic logs is in the order of a few node--hours.

% \ib{Should we drop this last paragraph? This artifact description should not be for "selling" our thing.}
% 
% The provided scripts and methodology [enable/facilitate] the community to evaluate the presented AI methods on different systems.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

This paper presents and evaluates a reinforcement learning~(RL) method that anticipates and triggers the mitigation of DRAM uncorrected errors.
The accompanying artifact provides all the code and data necessary for training and evaluation of this [RL?] method. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Software architecture}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Figure~\ref{fig:agent-and-environment}, included in the main manuscript, describes the RL~agent and its interaction with the environment: 


In our implementation based on historical logs, the environment obtains
the errors, events and job state from the logs, as described in
Section~\ref{}. In a real system, the environment would collect this information
from the monitoring daemons and workload manager. The
environment passes the state to the RL~agent, which supplies the state
features to the neural network to determine the action. 

Given
the action selected by the agent, the environment either performs a
mitigation or it does not. On the next event, it calculates the reward
for the last action, depending on the last time that mitigation was
performed and whether or not the next event is a UE.




\begin{itemize}
	\item \textbf{Environment}: encodes the features, UEs, and jobs derived from the logs and transfers this state information to the agent, which then performs an action. Following the agent's decision, the environment computes the reward (as described in Section~\ref{ssec:reward}) based on the mitigation and UE costs, and provides this feedback to the agent.
	\item \textbf{Agent}: supplies the state information given by the environment to the neural network, which subsequently determines whether the system should initiate a mitigation action. As described in Section~\ref{sec:background}, the agent employs two approaches during training: dueling double deep Q-network and prioritized experience replay.
\end{itemize}


	\item \textbf{Evaluation}: evaluates the performance of a model with the validation and test data.
	\item \textbf{Main}: creates the environment and the agent with the specified parameters, such as mitigation cost or time period. It then proceeds to train and evaluate the model.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Data models}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

